A conjugate subgradient algorithm with adaptive preconditioning for LASSO minimization

This paper describes a new efficient conjugate subgradient algorithm which minimizes a convex function containing a least squares fidelity term and an absolute value regularization term. This method is successfully applied to the inversion of ill-conditioned linear problems, in particular for computed tomography with the dictionary learning method. A comparison with other state-of-art methods shows a significant reduction of the number of iterations, which makes this algorithm appealing for practical use.

==> env_publi.tex <==
%
% NOTE : for iucr package, do not forget to put the option "pdf", 
%  otherwise figures won't display.
%
\usepackage{amsmath} %fleqn : align "equations" left
\usepackage{amsfonts}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{setspace} %setstretch
\renewcommand{\algorithmicrequire}{}
\renewcommand{\algorithmicensure}{\textbf{Output: }}
\usepackage{amssymb}
\usepackage{graphicx} %for includegraphics scaling
%\usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
\usepackage{fixltx2e}
%\usepackage{caption}
%\usepackage{subcaption}\captionsetup{compatibility=false}


\usepackage[caption=false]{subfig}



\newcommand{\pic}[3]
{
\begin{figure}
\caption{#3}
\includegraphics[scale=#1]{#2}
\end{figure}
}
\newcommand{\twocolumns}[4]{
\begin{minipage}{#1\linewidth}
#3
\end{minipage}\hfill
\begin{minipage}{#2\linewidth}
#4
\end{minipage}\textbf{\\[10pt]}
}
% Math
\newcommand{\diff}{\operatorname{d}\!}
\newcommand{\setR}{\mathbb{R}}
\newcommand{\setN}{\mathbb{N}}
\newcommand{\esp}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\Space}{$\phantom{grrr}$}
\newcommand{\argmin}[1]{\underset{#1}{\operatorname{argmin}} \; } %note : Argmin with a "A" means a set (several solutions) whilst "argmin" is a unique solution.
\newcommand{\Argmin}[1]{\underset{#1}{\operatorname{Argmin}} \; } %note : Argmin with a "A" means a set (several solutions) whilst "argmin" is a unique solution.
\newcommand{\argmax}[1]{\underset{#1}{\operatorname{argmax}} \; } %note : Argmin with a "A" means a set (several solutions) whilst "argmin" is a unique solution.
\let\oldvec\vec
\renewcommand{\vec}{\boldsymbol} %boldsymbol or mathbf ?
\newcommand{\tv}[1]{\operatorname{TV}\left( #1 \right)}
\newcommand{\prox}[2]{\operatorname{prox}_{#1}{\left(#2\right)}}
\newcommand{\proj}[2]{\operatorname{Proj}_{#1}{\left(#2\right)}}
\newcommand{\sign}[1]{\operatorname{sign}\left( #1 \right)}
\newcommand{\braket}[2]{\left\langle #1 \, , \, #2 \right\rangle}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\id}{\operatorname{Id}}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\lag}[1]{\mathcal{L}\left( #1 \right)}
\newcommand{\mmax}[2]{\max_{#1}\left\{ #2 \right\}}
\newcommand{\mmin}[2]{\min_{#1}\left\{ #2 \right\}}
\newcommand{\conv}{\ast} 
\newcommand{\ft}[1]{\mathcal{F}\left( #1 \right)}
\newcommand{\ift}[1]{\mathcal{F}^{-1}\left( #1 \right)}
\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\E}[1]{\cdot 10^{#1}} %notation scientifique. Utiliser "e", "E", ou "10^" ?
